Embedded Model Error Representation for Bayesian Model Calibration

Model error estimation remains one of the key challenges in uncertainty quantification and predictive science. For computational models of complex physical systems, model error, also known as structural error or model inadequacy, is often the largest contributor to the overall predictive uncertainty. This work builds on a recently developed framework of embedded, internal model correction, in order to represent and quantify structural errors, together with model parameters, within a Bayesian inference context. We focus specifically on a Polynomial Chaos representation with additive modification of existing model parameters, enabling a non-intrusive procedure for efficient approximate likelihood construction, model error estimation, and disambiguation of model and data errors' contributions to predictive uncertainty. The framework is demonstrated on several synthetic examples, as well as on a chemical ignition problem.

==> Makefile <==
SECTIONS = $(wildcard sections/*.tex)
FIGURES_TIKZ = $(shell find figs -type f -name '*.tikz')
FIGURES_TIKZ_PDF = $(FIGURES_TIKZ:%.tikz=%.pdf)
FIGURES_EPS = $(shell find figs -type f -name '*.eps')
FIGURES_EPS_PDF = $(FIGURES_EPS:%.eps=%-eps-converted-to.pdf)
FIGURES_ONLY_PDF = $(shell find figs -type f -name '*.pdf')

all: main.pdf

main.pdf: main.tex $(SECTIONS) $(FIGURES_TIKZ_PDF) $(FIGURES_EPS) \
	$(FIGURES_ONLY_PDF) local.bib
	latexmk -pdf -interaction=nonstopmode main.tex

$(FIGURES_TIKZ_PDF): %.pdf: %.tikz figures/header figures/footer
	cat figures/header $< figures/footer > figures/temp.tex;
	latexmk -pdf -interaction=nonstopmode -jobname=$(basename $@) figures/temp.tex

.PHONY: clean cleanmain cleanall

# You can choose which renegerable files you want to add or exclude below.
clean:
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.glo *.idx *.ilg *.ind *.lof *.log *.lot \
	      *.nav *.out *.ps *.snm *.spl *.toc
	@echo -n "Start cleaning tikz regenerable files..."
	@rm -f $(FIGURES_TIKZ:%.tikz=%.aux)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.bbl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.blg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.brf)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.dvi)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fdb_latexmk)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.fls)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.glo)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.idx)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ilg)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ind)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lof)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.log)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.lot)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.nav)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.out)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.ps)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.snm)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.spl)
	@rm -f $(FIGURES_TIKZ:%.tikz=%.toc)
	@echo "done."
	cd figures; rm -f temp.tex ;\
	rm -f *.aux *.bbl *.blg *.brf *.dvi *.fdb_latexmk \
	      *.fls *.idx *.ilg *.ind *.log *.out *.ps *.spl *.toc

cleanmain:
	@make clean
	rm -f main.pdf

cleanall:
	@make cleanmain
	@echo "Start cleaning tikz pdf files..."
	@rm -f $(FIGURES_TIKZ_PDF)
	@echo "done."
	@echo "Start cleaning eps pdf files..."
	@rm -f $(FIGURES_EPS_PDF)
	@echo "done."

